VLIS: Unimodal Language Models Guide Multimodal Language Generation

Multimodal language generation, which leverages the synergy of language and vision, is a rapidly expanding field. However, existing vision-language models face challenges in tasks that require complex linguistic understanding. To address this issue, we introduce Visual-Language models as Importance Sampling weights (VLIS), a novel framework that combines the visual conditioning capability of vision-language models with the language understanding of unimodal text-only language models without further training. It extracts pointwise mutual information of each image and text from a visual-language model and uses the value as an importance sampling weight to adjust the token likelihood from a text-only model. VLIS improves vision-language models on diverse tasks, including commonsense understanding (WHOOPS, OK-VQA, and ScienceQA) and complex text generation (Concadia, Image Paragraph Captioning, and ROCStories). Our results suggest that VLIS represents a promising new direction for multimodal language generation.

==> tables/story_table_backup.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{l|ccccc}
        % Models & rep-2 & rep-3 & rep-4 & div. & coh. & MAUVE & CLIPScore \\
        Models & rep-4 & div. & coh. & MAUVE & CLIP \\
        \hline
        %Greedy & 22.27 & 15.42 & 12.36 & 0.58 & 0.47 & 0.53 & 0.23 \\
        Greedy  & 12.36 & 0.58 & 0.47 & 0.53 & 0.23 \\
        %Beam & 26.76 & 21.79 & 18.85 & 0.47 & 0.48 & 0.46 & 0.25 \\
        Beam  & 18.85 & 0.47 & 0.48 & 0.46 & 0.25 \\
        % Top-K~\cite{} & 3.38 & 0.76 & 0.23 & 0.95 & 0.46 & 0.86 & 0.21 \\
        Top-K~\cite{} & 0.23 & 0.95 & 0.46 & 0.86 & 0.21 \\
        % Nucleus~\cite{} & 2.92 & 0.60 & 0.18 & 0.96 & 0.45 & 0.88 & 0.21 \\
        Nucleus~\cite{} & 0.18 & 0.96 & 0.45 & 0.88 & 0.21 \\
        % Typical-P~\cite{} & 2.52 & 0.46 & 0.12 & 0.97 & 0.45 & 0.84 & 0.19 \\
        Typical-P~\cite{} & 0.12 & 0.97 & 0.45 & 0.84 & 0.19 \\
        % Cont. Search~\cite{} & 2.49 & 0.38 & 0.09 & 0.97 & 0.49 & 0.89  & 0.28 \\
        Cont. Search~\cite{} & 0.09 & 0.97 & 0.49 & 0.89  & 0.28 \\
        %MAGIC~\cite{} & 2.51 & 0.38 & 0.09 & 0.97 & 0.51 & 0.91 & 0.36  \\
        MAGIC~\cite{} & 0.09 & 0.97 & 0.51 & 0.91 & 0.36  \\
        \hline
        Vanilla BLIP-2 & - & - & - & - & -  \\
        Naive Ensemble & - & - & - & - & -  \\
        \hline
        Ours & - & - & - & - & -  \\
        \hline
        Human & 0.09 & 0.97 & 0.54 & 1.00 & 0.40
        % Ours-opt-iml-max-30b & \checkmark & \checkmark & - & \textbf{34.6} 
    \end{tabular}
    \caption{Results in the ROCStories story generation dataset~\cite{}.}
    \label{tab:okvqa_table}
\end{table}
